DeepTracker: Visualizing the Training Process of Convolutional Neural Networks

Deep convolutional neural networks (CNNs) have achieved remarkable success in various fields. However, training an excellent CNN is practically a trial-and-error process that consumes a tremendous amount of time and computer resources. To accelerate the training process and reduce the number of trials, experts need to understand what has occurred in the training process and why the resulting CNN behaves as such. However, current popular training platforms, such as TensorFlow, only provide very little and general information, such as training/validation errors, which is far from enough to serve this purpose. To bridge this gap and help domain experts with their training tasks in a practical environment, we propose a visual analytics system, DeepTracker, to facilitate the exploration of the rich dynamics of CNN training processes and to identify the unusual patterns that are hidden behind the huge amount of training log. Specifically,we combine a hierarchical index mechanism and a set of hierarchical small multiples to help experts explore the entire training log from different levels of detail. We also introduce a novel cube-style visualization to reveal the complex correlations among multiple types of heterogeneous training data including neuron weights, validation images, and training iterations. Three case studies are conducted to demonstrate how DeepTracker provides its users with valuable knowledge in an industry-level CNN training process, namely in our case, training ResNet-50 on the ImageNet dataset. We show that our method can be easily applied to other state-of-the-art "very deep" CNN models.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

==> texfiles/acknowledgment.tex <==
%!TEX root = ../article.tex
% !TeX spellcheck = en_US

%% if specified like this the section will be committed in review mode
\acknowledgments{
	The authors want to thank xxx.
}

==> texfiles/reqanalysis.tex <==
%!TEX root = ../deeptracker.tex
% !TeX spellcheck = en_US

\section{Requirement Analysis}
\label{sec:requiments}

%This section first describes the data format dumped in the training process of CNNs. Subsequently, we discuss the design requirements.

\name was developed in approximately nine months, in which we collaborate closely with three experts (denoted by \ea, \eb, and \ec) who have considerable experience in CNNs. We held regular discussions with these experts once a week.

%\subsection{Data Abstraction}

%$L=\{l_{i}|i\in []  \}$
%All the experts show their desires to . Thus, 
From our regular discussions, we learned that the experts have to tune and fix a number of \textit{hyper-parameters} (learning rate, batch size, layer number, filter number per layer, weight decay, momentum, etc.) before starting a training trial.
These hyper-parameters, which strongly influence how a CNN is trained, are usually selected based on the experiences learned from their previous trials. 
%\dy{It is noted that, learning rate is a special hyper-parameter that can be changed during a training process. Typically, it is suggested to turn down the learning rate when the validation error rate and loss do not decrease anymore for a long time.}
After a training starts, the weights of each layer will be iteratively updated automatically, and the experts have little control over the updates.
At each iteration, the neuron weights are the key information that defines the network and training quality.
For example, the weights must approximately have a normal distribution after the first several iterations. 
Otherwise, it may indicate a problematic training caused by a high learning rate or insufficient regularization (e.g., weight decay). 
%Exploding or vanishing gradient values are also a bad sign for the training.
To track the change in performance across iterations, current popular training frameworks usually provide two pieces of summary information, namely, error rate and loss, on the training and validation datasets ($D_t$ and $D_v$).
The error rate indicates the percentage of mislabeled images, while the loss measures the prediction errors.
Typically, both error rate and loss should decrease over time. 
The increase of loss on $D_t$ may indicate an ill distribution of weights. 
A big gap between error rates of $D_t$ and $D_v$ may suggest the is over-fitting, while the absence of any gap may indicate that the model has a limited learning capacity.
These are some basic rules that the experts concluded from their numerous trials. 
However, the experts also encountered many phenomena that they could not explain or understand.
For example, when the global error rate remains stable, significant changes may still happen in some individual image classes. Sometimes there are significant changes in a few filters, which lead to a big impact on the performance on several classes. The experts desire to know which filters have the greatest influence on the performance changes of which classes.
These detailed changes obviously cannot be revealed via simple summaries, such as global error rate and loss.
Therefore, the feedback collected from these experts strongly suggests an urgent need to develop a visual system that allows them to interact with the complete training log data and explore multiple types of training behaviors. 
%During the process, current popular frameworks provide the experts with the basic statistical information of weight and gradients for each layers, which are useful for them to understand and debug the network.
%For example, for weights, it should have an approximately Gaussian (normal) distribution after several iterations. If there are weights that are diverging to very large positive or negative values, this may be caused by a high learning rate or insufficient regularization (e.g., weight decay). 
%For the gradient information, the experts should keep an eye out for exploding/vanishing values that indicate some problems may exist in current networks. There should be different statistical value scale or trend for different layers at different depths, the experts often need to compare them.
%In addition, there are two more types of values are important indicators for the experts to track the performance of a CNN, namely, the error rate and the loss on a given dataset ($\mathit{D_t}$ and $\mathit{D_v}$). The error rate is the percentage of images labeled incorrectly and the loss measures the prediction errors. Typically, both error rate and loss should (overall) go down over iterations. Increasing loss on $\mathit{D_t}$ can be indicative of some network issues such as, the high learning rate or incorrect data normalization.  A big gap between error rate of $\mathit{D_t}$ and $\mathit{D_v}$ may suggest the model is overfitting, while no gap may indicate the model has limited learning capacity.

%However, when the number of layers increase to tens or hundreds, it is becoming more and more challenging for the experts to efficiently find abnormals in layers, not mention to conducting comparison among such many layers. Moreover, only showing how single value like error rate or loss change over time hide the rich dynamics behind it. For example, sometimes even the error rate remain the same, there are some significant changes on some image classes.
%Therefore, the feedback collected by the all three experts strongly suggests that a visual system that enables analysts to interact with the complete training log data and explore training behavior is urgently needed. 

%\ww{maybe give a short paragraph explain how people visualize training in previous work or exiting framework, which is the training/validation error/loss, and what their meaning, and how important it is, and how people interpret them. then we can say our experts are not satisfy with them, because xxx, and then we have frequent discussion to dientify xxx...}



%\subsection{Requirement Analysis}


%After several rounds of structure interviews with the experts, we summarized and complied a list of design requirements as follows. 
We summarize and compile the following list of requirements after several rounds of structured interviews with the experts:

%Therefore, our focus is to design an informative and intuitive visualization interface for both real-time monitoring of a CNN performance and historical data analysis. In this manner, users can .

%Notice that the requirements are derived from the feedback of the experts, as well as the knowledge gleaned from the literature review. 

\begin{compactenum}[R.1]
	%\setcounter{enumi}{4}
	%\itemsep-0.1em 
	%\item \textbf{ xx }%Preserve the familiar forms for displaying the basic information}.
	%It is a fundamental task to show the model-performance-related information (i.e., the loss and error of training/validation ). Meanwhile, the learning rates 
	%showing the how learning rate variate over time.
	
	\item \textbf{Exploring multiple facets of neuron weight information}.
	A single iteration may have millions of weight updates, but individual values are generally meaningless to the experts.
	Instead, the experts are more interested in the statistical information of these weights at the layer and filter levels.
	All three experts emphasized the importance of intuitively examining and comparing general types of statistics, such as sum and variance, between these levels.
%	The layer-relevant information includes layer-level and filter-level statistical information. For the layer-level information, it contains various types of statistics, such as sum and var. All the experts emphasize the importance of using intuitive (i.e., easy to understand) visualization to show this different types of layer-level statistical information. %Further, due to the hierarchical structures on CONV layers, the experts demands to be able to see the aggregated. 
	Besides, \ea and \eb strongly desire to see the weight change degree for filters over iterations to identify which filters change dramatically at which iteration or how a filter changes across iterations.
	% identify the exact location of the current selected layer

%should be allowed to identify the specific value of a selected iteration, the trend over the entire training process, and positive and negative for a statistical information of a given layer. In addition, as there will be too many layers when using a very deep CNN (e.g., vgg-19 and resnet50),it is impossible to show all the layers directly. The system should provide a reasonable aggregation and interaction manner to allow the experts to explore the information they desired while not disturbed from other redundant information.\\
		
	\item \textbf{Comparing multiple layers}.
	All three experts like to compare layer-level statistical information. 
	For example, they want to know whether a specified measure of different layers show a similar trend or distribution (e.g., whether the sum is positive or negative).
	Accordingly, our visualization should also help these experts in performing such comparisons. 
	%Due to the great depth and the inner hierarchical structure of a very deep CNN (e.g., resnet50), the layer-relevant information. 
	%For example, the std of weight should be smaller for the layers with less neurons. Besides, knowing the differences and similarities among layers can help the experts gain more understanding about the function of layers.
		
	\item \textbf{Tracking the classification results of validation classes}.
	Validation is a critical step in the training process that ``test drives'' the trained CNN and tracks its performance change across iterations~\cite{bengio2012practical}.
	Previous tools only measure the global validation loss/error, thereby concealing the rich dynamics of how the image labels of each class change over time.
	%Previous tools only measure the global validation loss/error for comparison purposes.
	%Meanwhile, it also conceals the rich dynamics of how image labels of each class change over time.
	When the error rates do not reduce as expected, the experts find that such highly-aggregated information is useless and cannot help them understand why or when the training runs into a bottleneck.
	%Previous tools only provide the experts with high-level model performance information, namely, the validation loss and  error. It fails to disclose the detailed information about how the labels of images of each class change over the time. 
	Therefore, the experts want to know how the images of different classes behave differently and identify those classes that are easy or difficult to train.
	%Which classes of images are easy to identified correctly and which classes are difficult for classification. 

	\item \textbf{Detecting important iterations}.
	One complete training process usually contains millions of iterations, but it is obvious that not all iterations are equally important.	
	For example, some image classes may suddenly change their error rates after certain weight updates.
	The experts are interested in these patterns, which may help reveal in-depth relationships between filters and image features.
	However, the overall error rate trend does not help much, since it generally decreases slowly and steadily.
	Thus, the experts hope that our system can help them identify the abnormal iterations and the corresponding classes.
	
%	In the training process, although the overall accuracy to all images is always decreasing slowly and steadily, it does not hold true for the images of one class. The experts shows great interests on the iterations when the error of one or a set of classes may change significantly. The visual encoding should highlight these abnormal iterations and the corresponding classes.
	
	\item \textbf{Examining individual validation classes}.
	Our initial prototype shows that different classes clearly have different error rate evolution patterns. 
	%Thus, experts \eb and \ec are curious about those classes of poor performances, thereby desiring to further explore the image label information for these classes. 
	Thus, experts \eb and \ec are curious about those classes with very poor or excellent performance, thereby desiring to further explore the image label information for these classes. 
	For example, they want to see whether and why some images are always misclassified. 
	%such as what kind of images in this class are always labeled wrongly or rightly, which images are not in a stable status(i.e., sometimes labeled wrongly and sometimes labeled rightly), and what exactly happens in the detected important iteration.
	
	\item \textbf{Enabling correlation exploration}.
	Apart from analyzing the weight and validation data separately, the experts are also curious about their relational patterns.
	They are specifically interested in uncovering the relationships between the layers or filters and the validation images, such as how the changes in network parameters respond to the image labeling results for each class. 
	By connecting these two pieces of information together, they hope to gain fundamental insights into the behaviors of CNNs and to improve training results.
%	In particular, they want to figure out how the changes of network parameters respond to image labeling result for each class. They are especially interested in uncovering the relationships between the layers or filters and the images of each class. In other words, for a class of images, which layers or filters may have the greatest impacts on their labeling results.
%	Although the experts agree that analyzing the weight and validation data separately can offer the experts understanding about how a CNN is trained~\cite{bengio2012practical, rauber2017visualizing}, they show more interests on the correlation between the changes of layer-relevant statistical data and image labeling data, which is no studied in prior work. In particular, they want to figure out how the changes of network parameters respond to image labeling result for each class. They are especially interested in uncovering the relationships between the layers or filters and the images of each class. In other words, for a class of images, which layers or filters may have the greatest impacts on their labeling results.
\end{compactenum}




==> texfiles/viznetrain.tex <==
%!TEX root = ../article.tex
% !TeX spellcheck = en_US

\section{VizNeTrain\label{sec:visualization}}

visual design

1. hierarchical tree combining with small multiple time-series
   advantage:
  
2. header

\subsection{System Overview}
  1. development environment; 2. system architecture;

==> texfiles/viztrain.tex <==



We trained a large, deep convolutional neural network (resnet50 [x])to classify the 1.3 million high-resolution images in the  ImageNet LSVRC-2012 contest, which contains 1000 different classes and each class include 1,300 images.



Imagenet Large-Sc ale Visual Recognition Challenge 2012 (ILSVRC) contains roughly 1.3 million training images, 50,000 validation images.


Resnet164, cifar-10 dataset[] consists of 50k training images and 10k testing images in 10 classes. Our focus is on visualizing the behaviors of extremely deep networks, and compare the difference between networks whose layer number are not that crazy.
